The Farey graph is uniquely determined by its connectivity

We show that, up to minor-equivalence, the Farey graph is the unique minor-minimal graph that is infinitely edge-connected but such that every two vertices can be finitely separated.

==> FareyGraphDef.tex <==
A \emph{halved Farey graph} of \emph{order} $0$ is a $K^2$ whose sole edge is coloured blue.
Recursively, a \emph{halved Farey graph} of \emph{order} $n>0$ is an edge-coloured graph $G$ that is obtained from a halved Farey graph $H$ of order $n-1$ as follows.
The graph $G$ is obtained from $H$ by adding a new vertex $v_e$ for every blue edge $e$ of $H$ and joining $v_e$ precisely to the endvertices of $e$.
The edge-colouring of $G$ colours the new edges blue whereas all edges of $H\subset G$ receive black.
Since all halved Farey graphs of order $n$ are isomorphic to each other via isomorphisms that respect their edge-colourings, we speak of \emph{the} halved Farey graph $\hFG_n$ of order $n$ and assume that $\hFG_{n+1}$ arises from $\hFG_n$ as described above.
The \emph{halved Farey graph} is the union $\hFG:=\bigcup_{n\in\N}\hFG_n$ of all halved Farey graphs $\hFG_n$ of order~$n$, and it does not come with an edge-colouring.

The Farey graph is constructed quite similarly.
A \emph{Farey graph} of \emph{order} $0$ is a $K^2$ whose sole edge is coloured blue.
A \emph{Farey graph} of \emph{order} $1$ is obtained from a $C^4$ with blue edges by adding one black chord.
Recursively, a \emph{Farey graph} of \emph{order} $n>1$ is an edge-coloured graph $G$ that is obtained from a Farey graph $H$ of order $n-1$ as follows.
The graph $G$ is obtained from $H$ by adding a new vertex $v_e$ for every blue edge $e$ of $H$ and joining $v_e$ precisely to the endvertices of~$e$.
The edge-colouring of $G$ colours the new edges blue whereas all edges of $H\subset G$ receive black.
Again, we speak of \emph{the} Farey graph $F_n$ of order $n$.
The \emph{Farey graph} is the union $F:=\bigcup_{n\in\N}F_n$ of all Farey graphs $F_n$ of order~$n$.
Like the halved Farey graph, it does not come with an edge-colouring.
Note that the Farey graph can be obtained from two copies of the halved Farey graph by pasting them along $\hFG_0$.
This recursive construction of the Farey graph is based on~\cite{OfficeHoursGroupTheory}.

\begin{lemma}\label{FareyGisMinorOfHalvedFareyG}
The halved Farey graph and the Farey graph are minor-equivalent.
\end{lemma}
\begin{proof}
The halved Farey graph is a subgraph of the Farey graph.
Conversely, the Farey graph is a minor of the halved Farey graph: if $e$ is a blue edge of $\hFG_1$, then the Farey graph is the contraction minor of $\hFG-e$ whose sole non-trivial branch set is~$V(\hFG_0)=K^2$, i.e., $(\hFG-e)/V(\hFG_0)\cong\FG$.
\end{proof}

